Quality Control in Open-Ended Crowdsourcing: A Survey

Crowdsourcing provides a flexible approach for leveraging human intelligence to solve large-scale problems, gaining widespread acceptance in domains like intelligent information processing, social decision-making, and crowd ideation. However, the uncertainty of participants significantly compromises the answer quality, sparking substantial research interest. Existing surveys predominantly concentrate on quality control in Boolean tasks, which are generally formulated as simple label classification, ranking, or numerical prediction. Ubiquitous open-ended tasks like question-answering, translation, and semantic segmentation have not been sufficiently discussed. These tasks usually have large to infinite answer spaces and non-unique acceptable answers, posing significant challenges for quality assurance. This survey focuses on quality control methods applicable to open-ended tasks in crowdsourcing. We propose a two-tiered framework to categorize related works. The first tier introduces a holistic view of the quality model, encompassing key aspects like task, worker, answer, and system. The second tier refines the classification into more detailed categories, including quality dimensions, evaluation metrics, and design decisions, providing insights into the internal structures of the quality control framework in each aspect. We thoroughly investigate how these quality control methods are implemented in state-of-the-art works and discuss key challenges and potential future research directions.

==> 10Biography.tex <==
% 作者1图
% \begin{figure}[h]%
% \centering
% \includegraphics[width=0.3\textwidth]{First.eps}
% %\caption{First author}%\label{fig1}
% \end{figure}

%\begin{biography}
\noindent{\bf First Author} and the other authors may include
biographies at the end of the paper. The author's educational
background is listed. The degrees should be listed with type of
degree in what field, which institution, city, state or country, and
the year degree was earned. Listing military and work experience,
including summer and fellowship jobs at the end of this paragraph.
The current job must have a location.

The second paragraph uses the pronoun of the person (he or she) and
not the author$'$s last name. Information concerning previous
publications may be included. Try not to list more than three books
or published articles. The format for listing publishers of a book
within the biography is: title of book (city, state: publisher name,
year) similar to a reference. Current and previous research
interests should be stated.

The third paragraph begins with the author$'$s title and last name
(e.g., Dr. Smith, Prof. Jones, Mr. Kajor, Ms. Hunter). List any
memberships in professional societies. Finally, list any awards and
work for committees and publications. If a photograph (above 600
dpi) is provided, the biography will be indented around it. The
photograph is placed at the top left of the biography. Personal
hobbies will be deleted from the biography. Please see the following
example for more details.

E-mail: mir@ia.ac.cn (Corresponding author)

ORCID iD: 0000-0000-0000-0000




%\end{biography}

% 作者2图
% \begin{figure}[h]%
% \centering
% \includegraphics[width=0.3\textwidth]{Second.eps}
% %\caption{Second author}%\label{fig1}
% \end{figure}

%\begin{biography}
\noindent{\bf Second Author }\quad received the B.Sc. and M.Sc.
degrees in mechanical engineering from *** University, China in 1977
and 1984, respectively, and the Ph.D. degree in computing from ***
University, UK in 1992. In 1994, he was a faculty member at ***
University, China and in 1996 at *** University, USA. Currently, he
is a professor in Department of Information System Engineering at
*** University, China. Prof. Author received research award from
Science Foundation, and the Best Paper Award of the IS International
Conference in 2000 and 2006, respectively. He is a member of SICE,
IEE and IEEE.

His research interests include robotics, feedback control systems,
and control theory.

E-mail: mir@ia.ac.cn

ORCID iD: 0000-0000-0000-0000

%\end{biography}

% 作者3图
% \begin{figure}[h]%
% \centering
% \includegraphics[width=0.3\textwidth]{Third.eps}
% %\caption{Third author}%\label{fig1}
% \end{figure}

%\begin{biography}
\noindent{\bf Third Author }\quad received the B.Sc. and M.Sc.
degrees in mechanical engineering from *** University, China in 1977
and 1984, respectively, and the Ph.D. degree in computing from ***
University, UK in 1992. In 1994, he was a faculty member at ***
University, China and in 1996 at *** University, USA. Currently, he
is a professor in Department of Information System Engineering at
*** University, China. Prof. Author received research award from
Science Foundation, and the Best Paper Award of the IS International
Conference in 2000 and 2006, respectively. He is a member of SICE,
IEE and IEEE.

His research interests include robotics, feedback control systems,
and control theory.

E-mail: mir@ia.ac.cn

ORCID iD: 0000-0000-0000-0000

==> 8Conclusion.tex <==
\section{Conclusion}
\label{sec:con}

==> bib.tex <==
% \documentclass{article}
% \begin{document}
%     \nocite{*}
%     \bibliographystyle{fcs}
%     \bibliography{mybib}
% \end{document}
